Rumor Spreading with Bounded In-Degree

In the classic gossip-based model of communication for disseminating information in a network, in each time unit, every node $u$ is allowed to contact a single random neighbor $v$. If $u$ knows the data (rumor) to be disseminated, it disperses it to $v$ (known as PUSH) and if it does not, it requests it from $v$ (known as PULL). While in the classic gossip model, each node is only allowed to contact a single neighbor in each time unit, each node can possibly be contacted by many neighboring nodes. In the present paper, we consider a restricted model where at each node only one incoming request can be served. As long as only a single piece of information needs to be disseminated, this does not make a difference for push requests. It however has a significant effect on pull requests. In the paper, we therefore concentrate on this weaker pull version, which we call 'restricted pull'. We distinguish two versions of the restricted pull protocol depending on whether the request to be served among a set of pull requests at a given node is chosen adversarially or uniformly at random. As a first result, we prove an exponential separation between the two variants. We show that there are instances where if an adversary picks the request to be served, the restricted pull protocol requires a polynomial number of rounds whereas if the winning request is chosen uniformly at random, the restricted pull protocol only requires a polylogarithmic number of rounds to inform the whole network. Further, as the main technical contribution, we show that if the request to be served is chosen randomly, the slowdown of using restricted pull versus using the classic pull protocol can w.h.p. be upper bounded by $O(\Delta / \delta \log n)$, where $\Delta$ and $\delta$ are the largest and smallest degree of the network.

==> miscellaneous.tex <==
\section{Miscellaneous}
For other concepts of (partial) stochastic dominance consult (almost) \emph{Partial stochastic dominance by Kamihigashi and Stachurski, Kobe University}, e.g. let $X$ and $Y$ be $S$ valued random variables. Then $X$ stoch. dominates $Y$ iff
$$E(f(X))\geq E(f(Y)), \text{for all increasing functions $f:S\rightarrow \RR$} $$ 
A function $f:\S\rightarrow \RR$ is called increasing if $s_1\leq s_2$ implies $f(s_1)\leq f(s_2)$

\subsection*{Comments \& Todo}

\yannic{Case with $r-\rpull\ $ for $r>1$, e.g. $r=\log(n)$. How much can we improve?}

ALL THE THINGS GET EASIER IF WE HAVE $W\subseteq N^1(S)$ as we are only simulating one round of \pull. CHECK WHERE IT MIGHT GET EASIER. DO NOT


From the tree chapter:
\sebastian{
we have a whole bunch of things to look at:

choice model: adversary, random, det. (all restr.) vs. normal pull\\
(i'd prefer to leave out the deterministic version)\\
algo: only (r)pull or rather push/(r)pull\\
running time: in expectation (full graph/path - latter rather a tool for the former) vs. high probability\\

gives a total of about 4*2*2 different scenarios - though quite a few will collide.\\

Below so far:\\
adversary \& \rpull \& path, random \& \rpull \& path,\\
adversary \& \prp \& full tree, random \& \prp \& full tree,\\
adversary \& \rpull \& general graph, random \& \rpull \& general graph
}


\subsubsection{Some unimportant stuff}
Note that in this paper we consider \emph{acceptance choice} a model parameter, while in some cases it makes sense to give the nodes the power of deciding \emph{how} to choose which incoming request to accept. However, in such a case a requesting node $u$ must be allowed to send a small amount of information $I_{u,t}$ (like its \ID\ or some information it has gathered until time $t$) apart from the request, which can then be evaluated \emph{before} the requested node $v$ decides about whose request to accept. If such a node $v$ can actively decide which node it will take, it can choose by \ID, still at random or use a heuristic of its own, e.g. accepting the node that has made the least number of requests so far. Mathematically speaking, $v$ uses a function $f: (R, {\cal I}_t) \to V, (r, I_t) \mapsto u$, where $R$ is a set of random numbers/bit sequences and ${\cal I}_t$ is the power set of $\set{I_{v_1}, I_{v_2}, \dots, I_{v_n}}$, with $V=\set{v_1, \dots, v_n}$. 

\yannic{Is the last paragraph important?}
\sebastian{nope. but i preferred to have it written down somewhere, just in case we somehow want to make use of it at some point. we should kick it out later.}



I MOVED THE FOLLOWING FROM THE TREE CHAPTER. NO CLUE WHAT THIS WAS FOR. PLEASE COMMENT.

\paragraph{\prp\ on a tree.}
\yannic{Why do we do \prp\ all of a sudden?}
\begin{theorem}
\label{thm:pushPullTheorem}
  There is an instance for which \prp\ needs, \whp, $\Omega(n^{2/3})$ rounds in the adversarial RRS and $\bigO(n^{1/3})$ rounds in the random RRS.
\end{theorem}

% \input{picture-tree-pushrpull}

\begin{proof}
  \sebastian{that would be the part where we have that tree that is rooted at $r$, $r$ has many neighbors that block progress in both \push\ and \rpull, then one child has an edge to yet a copy of $r$ and that we can do couple of times, slowing the progress in the adversarial model}
  Consider the following $m$-parametrized tree $T_F(m)$. Define the following sets: $R=\set{r_1,\dots, r_m}$, $C=\set{c_1, \dots, c_m}$, $L_i=\set{l_{i,1}, l_{i,2}, \dots, l_{i,\alpha(m)}}$ and $L'_{i,j}=\set{l'_{i,j,1},\dots,l'_{i,j,\beta(m)}}$ for $i=1,\dots, m$ and $\alpha(m)=\Theta(m^?)$, $j=1,\dots,\alpha(m)$ and $\beta(m)=\Theta(\alpha(m)/\log n)$.  
For each $i$, edges go from $r_i$ to all nodes in $L_i$, and from all $l_{i,j}$ to all nodes in $L'_{i,j}$. Additionally, $r_i$ is connected to $c_i$ and for $i<m$, $c_i$ is connected to $r_{i+1}$. Thus we have a path $p_m=(r_1, c_i, r_2, c_2, \dots, c_m)$ and each $r_i$ is the root of a two-level subtree.

Let $S_0=\set{r_1}$. Consider a time $t_i$ such that $r_i$ just got informed in round $t-1$. Thus, all its children in $L_i$ are uninformed. Each round in which the information does not pass to $c_i$, it propagates to one node in $L_i$ via \push\ and to (at most ) one other node via \rpull. Thus, after $t$ further rounds, at most $2t$ of the nodes in $L_i$ are informed. For $t\leq\alpha(m)/4$, the probability that $r_i$ pushes the information to $c_i$ (assuming that it does not push to nodes that it previously forwarded the information to) is smaller than $2/\alpha(m)$. At the same time, even though $c_i$ requests from $r_i$ with probability $1/2$, each round an uninformed node $l_{i,j}$ requests from $r_i$ with probability $1/\beta(m)$, and since there are at least $\alpha(m)/2$ such nodes, \whp\ at least one of them requests at $r_i$, too, giving the adversary the possibility to postpone propagation along the path $p_m$. Each such round an \rpull\ request by $c_i$ is unsuccessful \whp, while a \push\ from $r_i$ does not reach $c_i$ with probability $1-2/\alpha(m)$ and we upper bound their joint event by $1-3/\alpha(m)$.

Let $T_i$ be the random variable that measures the amount of time needed for $c_i$ to get the message once $r_i$ gets informed. This random variable is upper bounded by a geometrical random variable $Geo(3/\alpha(m))$, which automatically succeeds after $\alpha(m)/3$ rounds, causing $\E[T_i]$ to be upper bounded by $\alpha(m)/4$ (i guess?). Summing up over all $T_i$ and using Chernoff we get a running time in the adversarial model of $\Omega(m\alpha(m))+\log n$ with high probability.

In the random model
\end{proof}





==> occupation_bound.tex <==
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
\input{header_and_tail_makros}
\includeHeader
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
%
\section{Bounds for Broadcast Time of Random \rpull}
\subsection{Occupation Bound}
%
%
Let $S$ be the set of informed nodes at the start of the algorithm, $U:= V \setminus S$ and let $\srv{S}^{\pull}_t$, $\srv{S}^{\rpull}_t$ be the random variables describing the set of informed nodes after $t \in \mathbb{N}$ rounds of \pull\ respectively \rpull\ both starting at $\srv{S}^{\pull}_0 = \srv{S}^{\rpull}_0 = S$. 

For any round $t \in \mathbb{N}$, node $w \in U$, $W\subset U$ and $R \subset S$ 
let $w \rightarrow_t R$ be the event describing that $w$ sends a request to a node in $R$ in round $t$. The other way round $w \leftarrow_t R$ means that $w$ gets informed by a node in $R$. Also, $W \leftarrow_t R$ happens if all nodes in $W$ get the information from a node in $S$, always referring to round $t$. The index $t$ is omitted if it does not lead to ambiguities.
For $t_0 \in \mathbb{N}$ let $B(w,R,t_0) \in \cb{0, 1}$ be the random variable with $B(w,R,t_0) = 1$ iff there is a round $t \leq t_0$ where $w \leftarrow_t R$ is true. Define the number of occupations of $W$ in $R$ as the random variable $B(W,R,t_0) := \sum_{w \in W} B(w,R,t_0)$. 

Let $u \in U$.
Define the set of informed neighbors $S_u := S \cap N(u)$ and the set of dependent uninformed nodes $U_u:=U \cap N(S_u)$, where $N(S_u) := \bigcup_{v\in S_u} N(v)$. 
Define $\srv{W}_u := \srv{S}^{\pull}_1 \cap U_u$.
We want to show an upper bound on $B := B(\srv{W}_u,S_u,t_0)$.

For simplicity we assume a certain symmetry of the graph, i.e., 
\begin{align*}
\forall v \in S_u: d(v) &= const \\
\forall w \in U_u: d(w) &= const \\
d_S(w) &= const \\
d_{S_u}(w) &= const
\end{align*}

We assume that we have only good rounds, i.e., $\forall v \in S: \rv{Q_v} \in \bigOOf{\frac{\Delta}{\delta} + \log(n)}$ \whp .
For $t_0 \in \omegaOf{\frac{\Delta}{\delta} + \log(n)}$, $v \in S_u$ and $w \in \srv{W}_u$ we show that
\begin{enumerate}[label=(\roman*)]
\item \label{itm:success_prob}
$\PrOf{w \leftarrow S_u \mid w \rightarrow S_u} \in \ThetaOf{\frac{d(w)}{d(v)}}$
\item \label{itm:Su_vs_S_ratio}
$\PrOf{w \leftarrow S_u \mid w \leftarrow S} \in  \ThetaOf{\frac{\Delta}{\delta} \frac{d_{S_u}(w)}{d_S(w)} \PrOf{w \leftarrow S_u \mid w \rightarrow S_u}}$
\item \label{itm:good_dependency}
$\PrOf{w \leftarrow S_u \mid \srv{W}_u \leftarrow S} \in  \ThetaOf{\PrOf{w \leftarrow S_u \mid w \leftarrow S}}$
\item \label{itm:cardW}
$\EOf{\card{\srv{W}_u}} \in \bigOOf{\frac{d(v)}{d_{S_u}(w)}\frac{d_S(w)}{d(w)}\card{S_u}}$
\item \label{itm:EofB_vs_cardW}
$\EOf{B \mid \srv{W}_u \leftarrow S} \in \ThetaOf{\card{\srv{W}_u} \PrOf{w \leftarrow S_u \mid \srv{W}_u \leftarrow S}}$
\item \label{itm:composition}
$\EOf{B \mid \srv{W}_u \leftarrow S} \in \bigOOf{\frac{\Delta}{\delta} \card{S_u}}$
\item \label{itm:whp}
$B \in \bigOOf{\frac{\Delta}{\delta} \card{S_u} + \log(n)} $ \whp given $\srv{W}_u \leftarrow S$
\end{enumerate}
and conclude for arbitrary values of $\card{\srv{W}_u}$
\begin{equation*}
B \in \bigOOf{\frac{\Delta}{\delta} \card{S_u} + \log(n)} \mbox{ \whp given }\srv{W}_u \subset \srv{S}^{\rpull}_{t_0}
\end{equation*}
%
%
%
\begin{proof}
%
\ref{itm:success_prob}
\begin{equation*}
\rv{X} \sim binom(m, p) \Rightarrow \EOf{(\rv{X} + 1)^{-1}} = (p(m+1))^{-1} \br{1 - \br{1-p}^{m+1}} \leq (p(m+1))^{-1}
\end{equation*}
%
Reference: Chao, M. T. \& W. E. Strawderman 1972. "Negative moments of
positive random variables". Journal of the American Statistical
Society, 67:429-431. \christof{see literature/Inverse\_Moments\_of\_Binomial\_Variates.pdf in the last part of introduction; did not find original paper (for free)}
%
Use $m = d(v)-1$ and $p^{-1} = d(w)$ to get $\PrOf{w \leftarrow S_u \mid w \rightarrow S_u} = \EOf{\rv{Q}^{-1}_v} \leq \frac{d(w)}{d(v)}$ where $\rv{Q}_v$ is the number of incoming requests on a node $v \in S_u$ in round $t$.

\ref{itm:Su_vs_S_ratio}
\begin{align*}
&
\PrOf{w \leftarrow S_u \mid w \leftarrow S} 
\\
&=
\frac{\PrOf{w \leftarrow S_u}}{\PrOf{w \leftarrow S}}
\\
&=
\frac{\PrOf{w \rightarrow S_u}\PrOf{w \leftarrow S_u \mid w \rightarrow S_u}}{\PrOf{w \rightarrow S}\PrOf{w \leftarrow S \mid w \rightarrow S}}
\\
&\leq 
\frac{\frac{d_{S_u}(w)}{d(w)} \PrOf{w \leftarrow S_u \mid w \rightarrow S_u}}{\frac{d_{S}(w)}{d(w)} \frac{\delta}{2 \Delta}}
\\
& \in
\bigOOf{\frac{\Delta}{\delta} \frac{d_{S_u}(w)}{d_S(w)} \PrOf{w \leftarrow S_u \mid w \rightarrow S_u}}
\end{align*}

\ref{itm:good_dependency}
Because all nodes in $\srv{W}_u$ are symmetric, their ratio of getting informed by $S_u$ vs $S$ is equal to $w$'s ratio. Thus, depending on $\srv{W}_u \leftarrow S$ instead of $w \leftarrow S$ cannot change the probability of $w \leftarrow S_u$ significantly as long as $\card{\srv{W}_u} \in \smallOOf{\card{S \cap N(W)} t_0}$. Otherwise the nodes in $\srv{W}_u$ would occupy nearly all of their informed neighbors $S \cap N(\srv{W}_u)$ in nearly every round $t < t_0$ and eventually reducing the number of free nodes to $\bigOOf{1}$. Then the ratio may change due to rounding effects. 
Because we assume that we have a good round, we know that the number of requests on a single node is in $\bigOOf{\frac{\Delta}{\delta} + \log(n)}$ \whp . This leads to $\card{\srv{W}_u} \in \bigOOf{\card{S \cap N(\srv{W}_u)} \br{\frac{\Delta}{\delta} + \log(n)}}$. Together with $t_0 \in \omegaOf{\frac{\Delta}{\delta} + \log(n)}$ we assure that we avoid the problem above. 

\ref{itm:cardW}
Obviously, the number of edges from $U_u$ to $S_u$ is bounded by the sum of degrees of the nodes in $S_u$, i.e., $\card{U_u} d_{S_u}(w) \leq \card{S_u} d(v)$. For \pull\ every node in $U_u$ has probability $\frac{d_S(w)}{d(w)}$, hence, we get $\EOf{\card{\srv{W}_u}} = \card{U_u} \frac{d_S(w)}{d(w)}$. Together with the inequality above we achieve the claimed result.

\ref{itm:EofB_vs_cardW}
The expectation of occupations is the sum over the probability of a node in $W$ to occupy a node in $S_u$.

\ref{itm:composition}
Use \ref{itm:success_prob}, \ref{itm:Su_vs_S_ratio}, \ref{itm:good_dependency} and \ref{itm:cardW} to get 
\begin{align*}
\EOf{\card{\srv{W}_u}} \PrOf{w \leftarrow S_u \mid \srv{W}_u \leftarrow S}
&\in 
\bigOOf{ \frac{d(v)}{d_{S_u}(w)} \frac{d_S(w)}{d(w)}\card{S_u} \frac{\Delta}{\delta} \frac{d_{S_u}(w)}{d_S(w)} \frac{d(w)}{d(v)} } 
\\&= 
\bigOOf{\card{S_u} \frac{\Delta}{\delta}} 
\end{align*}
Now the claim results from \ref{itm:EofB_vs_cardW}.
 
\ref{itm:whp}
$B = \sum_{w \in \srv{W}_u} B(w,S_u,t_0)$, $B(w,S_u,t_0)$ are negatively correlated, use
Chernoff
%
\end{proof}
%
%
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
\includeTail
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> packages.tex <==
% encoding of this file
\usepackage[utf8]{inputenc}
\usepackage{lmodern}
%
\usepackage{geometry}
%\usepackage{fullpage}
%\textwidth 6.5in
%\textheight 9in
%\baselineskip 13.2pt

\usepackage{amsmath, amsthm, amssymb}
\usepackage{mathtools}
\usepackage{cite}
\usepackage{url}

%\usepackage{cleveref}
\usepackage{hyperref} % hyperlinks on \ref{...} in PDF

\usepackage{appendix}
\usepackage{graphicx}
\usepackage{epstopdf}
%\usepackage{setspace}
\usepackage{enumerate}
\usepackage{color}
\usepackage{xcolor}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
%\usepackage{float}
\usepackage{multirow}
\usepackage{paralist}
%\usepackage{times}

%\usepackage{caption}
\usepackage{xspace}
%\usepackage{mdwlist}

\usepackage{enumitem}
\usepackage{nicefrac} % nice looking fractions in running text

% tikz
\usepackage{ifthen}
\usepackage{arrayjobx}
\usepackage{tikz}
\usetikzlibrary{positioning,decorations.pathreplacing}


==> preliminaries.tex <==
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
\input{header_and_tail_makros}
\includeHeader
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------

\section{Preliminaries}
\label{sec:preliminaries}

\paragraph{Network Model.} We model our network as an undirected graph $G=(V,E)$ of $n=|V|$ nodes. We write $N(v)$ for the neighbors of node $v$ and $d(v)=|N(v)|$ denotes the degree of $v$. For a set $S \subseteq V$ we write $N_S(v)=\set{u \in S: \set{u,v} \in E}$ for the neighbors of $v$ in $S$ and $d_S(v) := |N_S(v)|$ is $v$'s \emph{degree in $S$}. For $S\subseteq V$ we define $N(S)=\cup_{s\in S}N(s)$. For $V' \subseteq V$ we use the notation $G[V']$ to denote the subgraph of $G$ induced by node set $V'$.
%For the neighbors of a node $v$ in some set $S \subseteq V$ we use the notation $N_S(v)=\set{u \in S: \set{u,v} \in E}$ and $d_S(v) := |N_S(v)|$ denotes the degree of node $v$ in $S\subseteq V$; if $S=V$,  $d(v)$ denotes the degree of $v$. 
We denote by $\delta$ and $\Delta$ the minimal resp. maximal degree within the graph. Time is divided into synchronized rounds, but nodes do not have access to a global clock; yet we assume all nodes to start executing the corresponding rumor spreading algorithm in round $1$.

\paragraph{Restricted Rumor Spreading (RRS).} To communicate, in each round a node $u$ can request one connection to one neighbor $v$ in $N(u)$, which either accepts or ignores that request. As a newly investigated model assumption, we limit the number of requests a single node can accept each round to one.\\
If a request is accepted, a communication link is created and both involved nodes can exchange information. Note that we assume in this paper that a requesting node $u$ can not send any information before a communication link is created, more specifically, the requested node $v$ does not learn of $u$'s \ID, nor of any other information about $u$, unless it accepts $u$'s request. \sebastian{is this true at all?}

\paragraph{\boldpull:} In the widely researched algorithm \pull\ a set of nodes $S \subset V$ has some information, which the other nodes $U := V \setminus S$ do not know, but they know of this information's existence. To learn of that information, a node $u \in U$ selects one of its neighbors $v$ (usually chosen randomly) and requests the information in the hope that $v$ has it. In the standard models there is no limit to how many requests a node $v$ can accept and thus $u$ will either learn the information (if $v \in S$) or it learns that $v$ does not yet have the information ($v \in U$). 

\paragraph{\boldrpull:} In our model, $v$ can accept at most one request per round, thus, if $u$ requests from $v$, $v$ might ignore it in favor of accepting the request of another node $u' \in N(v) \cap U$. In this case $u$ does not learn whether $v \in S$ or $v \in U$.\\
To measure progress, we denote with $S=S_0$ the initial set of informed nodes and with $S_t$, $t\geq 0$ the set of informed nodes after $t$ time steps. $U_t$ is defined analogously. For randomized rumor spreading algorithms $S_t$ and $U_t$ are set valued random variables. \sebastian{we might want to work on that}

\paragraph{Acceptance choice.} In this paper we look at two different ways of how a node $v$ with multiple requests chooses which request to accept. In the \emph{adversarial RRS}, an adversary chooses which of the requesting neighbors of $v$ is accepted. In the \emph{random RRS} $v$ makes that choice uniformly at random.


% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
\includeTail
% ------------------------------------------------------------------------------
% ------------------------------------------------------------------------------
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

